Lax-Oleinik-type formulas and efficient algorithms for certain high-dimensional optimal control problems

Two of the main challenges in optimal control are solving problems with state-dependent running costs and developing efficient numerical solvers that are computationally tractable in high dimension. In this paper, we provide analytical solutions to certain optimal control problems whose running cost depends on the state variable and with constraints on the control. We also provide Lax-Oleinik-type representation formulas for the corresponding Hamilton-Jacobi partial differential equations with state-dependent Hamiltonians. Additionally, we present an efficient, grid-free numerical solver based on our representation formulas, which is shown to scale linearly with the state dimension, and thus, to overcome the curse of dimensionality. Using existing optimization methods and the min-plus technique, we extend our numerical solvers to address more general classes of convex and nonconvex initial costs. We demonstrate the capabilities of our numerical solvers using implementations on a central processing unit (CPU) and a field-programmable gate array (FPGA). In several cases, our FPGA implementation obtains over a 10 times speedup compared to the CPU, which demonstrates the promising performance boosts FPGAs can achieve. Our numerical results show that our solvers have the potential to serve as a building block for solving broader classes of high-dimensional optimal control problems in real-time.

==> ADMMcomp_HJ2.tex <==
\section{Some computations for the numerical implementations}\label{sec: ADMMcomp_HJ2}




 
\subsection{A numerical method for computing the proximal point of $u\mapsto \valuefn(x,t;u,a,b)$}
Here, we discuss how our update equation for $d_i^{k+1}$ in~\eqref{eqt: ADMM_HJ2_dupdate} is computed explicitly. For simplicity of notation, we drop the index $i$ as it will be well-understood that all quantities are one-dimensional and denote $c^k := v_i^{k+1} + \admmb_i^k$,
so that Equation (\ref{eqt: ADMM_HJ2_dupdate}) becomes
\begin{equation}\label{eqt: ADMM_HJ2_di_update_simplified}
    d^{k+1} = \argmin_{u\in\mathbb{R}} \left\{\valuefn(x,t; u,a,b) + \frac{\lambda}{2}(u - c^k)^2\right\}.
\end{equation}
We will now compute the minimizer $d^{k+1}$ of (\ref{eqt: ADMM_HJ2_di_update_simplified}) explicitly.
If $u \geq 0$, after some computation, the objective function in~\eqref{eqt: ADMM_HJ2_di_update_simplified} can be written as
\begin{align} 
    F(u;x,t,a,b) & := \valuefn(x,t; u,a,b) + \frac{\lambda}{2}(u - c^k)^2 \\
    & = \begin{dcases}
        \frac{u^3}{6b} + \frac{x^3}{6a} - \left(\frac{1}{6a} + \frac{1}{6b}\right)\left(\frac{au + bx - abt}{a+b}\right)^3 + \frac{\lambda}{2}(u - c^k)^2 & u\in \Omega_1(x,t,a,b),\\
        \frac{u^3}{6b} + \frac{x^3}{6a} + \frac{\lambda}{2}(u - c^k)^2 & u\in \Omega_2(x,t,a,b),\\ 
        \frac{u^3}{6b} - \frac{x^3}{6b} + \frac{\lambda}{2}(u - c^k)^2 & u\in \Omega_3(x,t,a,b),\\
        +\infty & \text{otherwise},
    \end{dcases}\label{eqt:appendixB_fnF_upos}
\end{align}
where the three regions $\Omega_1(x,t,a,b), \Omega_2(x,t,a,b), \Omega_3(x,t,a,b)\subset [0,+\infty)$ are defined by
\begin{equation}\label{eqt: ADMM_regions}
\begin{split}
    \Omega_1(x,t,a,b) &:= \left\{u\in (bt,+\infty)\colon x-at\leq u\leq x+bt\right\} \bigcup \left\{u\in[0,bt]\colon u\geq x-at,\,\, u\geq bt-\frac{bx}{a}\right\},\\
    \Omega_2(x,t,a,b) &:= \begin{dcases}
    \left[0,bt-\frac{bx}{a}\right) & x\geq 0, \\
    \emptyset & x<0,
    \end{dcases}\\
    \Omega_3(x,t,a,b) &:= \begin{dcases}
    [0,x+bt] & x\leq 0,\\
    \emptyset & x>0.
    \end{dcases}
\end{split}
\end{equation}

For $u \geq 0$, the derivative of $F$ with respect to $u$ is given by
\begin{equation}\label{eqt:appendixB_der1}
    \frac{\partial}{\partial u} F(u;x,t,a,b) = \begin{dcases}
        \frac{(2a+b)u^2 - 2a(x-at)u - b(x-at)^2}{2(a+b)^2} + \lambda (u - c^k) & u\in \Omega_1(x,t,a,b),\\
        \frac{u^2}{2b} + \lambda(u - c^k) & u\in \Omega_2(x,t,a,b) \cup \Omega_3(x,t,a,b),
    \end{dcases}
\end{equation}
and the second derivative of $F$ with respect to $u$ can be easily computed using \eqref{eqt:lemA2_pf_2der_om1} and \eqref{eqt:lemA2_pf_2der_om2}, for different cases. If $u < 0$, after some computation, the objective function in~\eqref{eqt: ADMM_HJ2_di_update_simplified} can be written as
\begin{align*}
    F(u;x,t,a,b) & := \valuefn(x,t; u,a,b) + \frac{\lambda}{2}(u - c^k)^2 \\
    & = \valuefn(-x,t; -u,b,a) + \frac{\lambda}{2}(u - c^k)^2 \\
    & = \begin{dcases}
        -\frac{u^3}{6a} - \frac{x^3}{6b} + \left(\frac{1}{6a} + \frac{1}{6b}\right)\left(\frac{bu + ax + abt}{a+b}\right)^3 + \frac{\lambda}{2}(u - c^k)^2 & -u\in \Omega_1(-x,t,b,a),\\
        -\frac{u^3}{6a} - \frac{x^3}{6b} + \frac{\lambda}{2}(u - c^k)^2 & -u\in \Omega_2(-x,t,b,a),\\ 
        -\frac{u^3}{6a} + \frac{x^3}{6a} + \frac{\lambda}{2}(u - c^k)^2 & -u\in \Omega_3(-x,t,b,a),\\
        +\infty & \text{otherwise}.
    \end{dcases}
\end{align*}
Thus, for $u < 0$, the derivative of $F$ with respect to $u$ is given by
\begin{equation}\label{eqt:appendixB_der2}
    \frac{\partial}{\partial u} F(u;x,t,a,b) = \begin{dcases}
        \frac{-(a+2b)u^2 + 2b(x+bt)u + a(x+bt)^2}{2(a+b)^2} + \lambda (u - c^k) & -u\in \Omega_1(-x,t,b,a),\\
        -\frac{u^2}{2a} + \lambda(u - c^k) & -u\in \Omega_2(-x,t,b,a) \cup \Omega_3(-x,t,b,a).
    \end{dcases}
\end{equation}
Note that the objective function $F$ is strictly convex and twice continuously differentiable with respect to $u$ by Lemma~\ref{lem: appendix_conv_S_x0}. Then, by the first and second derivative tests, the minimizer $d^{k+1}$ in~\eqref{eqt: ADMM_HJ2_di_update_simplified} is computed as follows
\begin{equation}\label{eqt: ADMM_dk_explicit_formula}
d^{k+1} =  
\argmin_{u\in\{u_1,u_2,u'_1,u'_2,x - at, x+bt\}} F(u;x,t,a,b)
\end{equation}
where
$u_1$, $u_2$, $u_1'$, $u_2'$ are the scalars defined by (if their corresponding right-hand side is a real number)
\begin{equation}
\begin{split}
    u_1 & := \frac{-(\lambda(a+b)^2 - a(x-at)) + \sqrt{(\lambda(a+b)^2-a(x-at))^2 + (2a+b)(b(x-at)^2 + 2\lambda c^k(a+b)^2)}}{2a+b}\\
    &= -\frac{\lambda(a+b)^2 - a(x-at)}{2a+b} + \sqrt{\left(\frac{\lambda(a+b)^2-a(x-at)}{2a+b}\right)^2 + \frac{b(x-at)^2}{2a+b} + \frac{2\lambda (a+b)^2c^k}{2a+b}},\\
    u_2 & := -\lambda b + \sqrt{(\lambda b)^2 + 2 \lambda b c^k}, \\
    u_1' & := \frac{\lambda(a+b)^2 + b(x+bt) - \sqrt{(\lambda(a+b)^2 + b(x+bt))^2 + (a+2b)(a(x+bt)^2 - 2\lambda c^k(a+b)^2)}}{a+2b}\\
    &= \frac{\lambda(a+b)^2 + b(x+bt)}{a+2b} - \sqrt{\left(\frac{\lambda(a+b)^2 + b(x+bt)}{a+2b}\right)^2 + \frac{a(x+bt)^2}{a+2b} - \frac{2\lambda (a+b)^2c^k}{a+2b}}, \\
    u_2' & := \lambda a - \sqrt{(\lambda a)^2 - 2\lambda a c^k}.
\end{split}
\end{equation}
If any point in $\{u_1, u_2,u'_1,u'_2\}$ is not well-defined, then we set it to be any point in $[x-at,x+bt]$ in~\eqref{eqt: ADMM_dk_explicit_formula}. 
Here, $u_1$ and $u_2$ are the roots of the first-order derivatives of $F$ given in the first and second lines of~\eqref{eqt:appendixB_der1}, respectively, at which the second-order derivative $\frac{\partial^2}{\partial u^2} F(u;x,t,a,b)$ is positive. Similarly, $u'_1$ and $u'_2$ are the roots of the first-order derivatives of $F$ given in the first and second lines of~\eqref{eqt:appendixB_der2}, at which the second-order derivative $\frac{\partial^2}{\partial u^2} F(u;x,t,a,b)$ is positive. 


Note that there are some similarities in $u_1$, $u_2$, $u_1'$ and $u_2'$. Denote each $u_i$ and $u_i'$ by $u_i(x,t,a,b,c^k)$ and $u_i'(x,t,a,b,c^k)$. Then, we have
\begin{equation*}
    u_i'(x,t,a,b,c^k) = -u_i(-x,t,b,a,-c^k).
\end{equation*}

Finally, we note that in practice, some care must be given to the implementation of updating $d^{k+1}$ using \eqref{eqt: ADMM_dk_explicit_formula} with regard to numerical accuracy. For example, tolerances may be required in numerically defining the inequalities in regions $\Omega_1(x,t,a,b),$ $\Omega_2(x,t,a,b),$ and $\Omega_3(x,t,a,b)$, as defined by \eqref{eqt: ADMM_regions}, so that no candidate minimizer $u_1, u_2, u_1', u_2'$ is erroneously disregarded. Alternatively, if multiple of $u_1, u_2, u_1', u_2'$ are well-defined and numerically lie in the appropriate region, then the corresponding values of $F$ may need to be compared, so that the correct minimizer is chosen.




\subsection{An equivalent expression for $\valuefn(x,t;u,a,b)$ and $\opttraj(s;x,t,u,a,b)$}
Let $\valuefn$ be the function defined by~\eqref{eqt: result_S2_1d} and~\eqref{eqt: result_S2_1d_negative}, and let $\opttraj$ is the function defined 
by~\eqref{eqt: optctrl2_defx_1},~\eqref{eqt: optctrl2_defx_2},~\eqref{eqt: optctrl2_defx_3}, and~\eqref{eqt: optctrl2_defx_neg} for different cases.
Now, we present an equivalent expression for $\valuefn$ and $\opttraj$, which is used in our implementation.

By straightforward calculation, the function $\valuefn$ can be expressed as
\begin{equation*}
    \valuefn(x,t;u,a,b) = 
    \begin{dcases}
    \max\{\valuefn_3(x,t;u,a,b), \min\{\valuefn_1(x,t;u,a,b), \valuefn_2(x,t;u,a,b)\}\} & \text{if } u\in [0, x+bt],\\
    \max\{\valuefn_3(-x,t;-u,b,a), \min\{\valuefn_1(-x,t;-u,b,a), \valuefn_2(-x,t;-u,b,a)\}\} 
    & \text{if } u\in [x-at, 0),\\
    +\infty &\text{otherwise},
    \end{dcases}
\end{equation*}
where $\valuefn_1,\valuefn_2$ and $\valuefn_3$ are the functions in the first, second, and third lines of~\eqref{eqt: result_S2_1d}, respectively.

Similarly, assuming $u\in [x-at,x+bt]$ holds, the function $\opttraj$ can be expressed as
\begin{equation*}
    \opttraj(s;x,t,u,a,b)
    = \begin{dcases}
    \max\{u-bs, a(s-t)+x,0\} & \text{if } x\geq 0, 0\leq u\leq x+bt,\\
    \max\{u-bs,0\} + \min\{-b(s-t)+x,0\}
    & \text{if } x< 0, 0\leq u\leq x+bt,\\
    \min\{u+as, -b(s-t)+x,0\} & \text{if } x< 0, x-at\leq u<0,\\
    \min\{u+as,0\} + \max\{a(s-t)+x,0\}
    & \text{if } x\geq 0, x-at\leq u<0.
    \end{dcases}
\end{equation*}
